Relational to RDF Data Exchange in Presence of a Shape Expression Schema

We study the relational to RDF data exchange problem, where the tar- get constraints are specified using Shape Expression schema (ShEx). We investi- gate two fundamental problems: 1) consistency which is checking for a given data exchange setting whether there always exists a solution for any source instance, and 2) constructing a universal solution which is a solution that represents the space of all solutions. We propose to use typed IRI constructors in source-to- target tuple generating dependencies to create the IRIs of the RDF graph from the values in the relational instance, and we translate ShEx into a set of target dependencies. We also identify data exchange settings that are key covered, a property that is decidable and guarantees consistency. Furthermore, we show that this property is a sufficient and necessary condition for the existence of universal solutions for a practical subclass of weakly-recursive ShEx.

==> app-data-exchange.tex <==
\section{Proofs of Theorems~\ref{} and \ref{}}
\label{app:data-exchange}
\subsection{Homomorphism in Formulas}
We define a mapping $h^F$ that will be used to define the notion of homomorphism from a formula into an instance. We use the notion of this homomorphism for chase purposes.
%We start by defining homomorphism between instances and homomorphism from a formula into an instance.
Let $\Fsig$ be a function signature and $F$ be an interpretation of $\Fsig$.
For a term $t$ over $\Fsig$ and a mapping $h: \Vars \to \Dom$, we define $h^F(t)$ as:
$$
h^F(t) =
\begin{cases}
  h(x) & \text{ if } t = x \in \Vars\\
  a & \text{ if } t = a \in \Dom\\
  f(h^F(\vect{t'})) & \text{ if } t = f(\vect{t'}) \text{ is a function term}.
\end{cases}
$$
The mapping $h^F$ is extended on atoms and conjunctions of atoms as expected: $h^F(R(\vect{t})) = R(h^F(\vect{t}))$ and $h^F(\bigwedge_{i \in 1..k} R_i(\vect{t}_i)) = \bigwedge_{i \in 1..k}h^F(R_i(\vect{t}_i))$.
Note that if the argument of $h^F$ does not contain function terms, the interpretation $F$ is irrelevant so we allow to omit the $F$ superscript and write e.g. $h(\vect{t})$ instead of $h^F(\vect{t})$.

A \emph{homomorphism} $h: \phi \to \Model$ between the conjunction of atoms $\phi$ over signature $\FOsig = \Rsig \cup \Fsig$ and the model $\Model = \Inst \cup F$ of $\FOsig$ is a mapping from $\fvars(\phi)$ to $\Dom$ s.t. for every atom $R(\vect{t})$ in $\phi$ it holds that $R(h^F(\vect{t}))$ is a fact in $\Inst$, where $\Inst$, resp. $F$, is the restriction of $\Model$ to $\Rsig$, resp. to $\Fsig$.

Remark that if $\phi$ does not contain function terms, then $F$ in the above definition is irrelevant and we write $h: \phi \to \Inst$ instead of $h: \phi \to \Model$ and $h(\vect{t})$ instead of $h^F(\vect{t})$.



==> extra.tex <==
\joseinline{ We say that $\DES$ is \emph{decomposed} if 1) only binary relation
  symbols are used in the source database schema, and 2) each binary relation
  can be constrained by a single key dependency with the first attribute being
  the key. $\DES$ is \emph{strongly-typed} if for every type $T$ defined in
  $\ShexSch$ there is a skolem function symbol $f_T$ in $\Fsig$, its
  interpretation $f_T^{\Fint}$ is injective, and furthermore, its range is
  disjoint with the range of the interpretation $f_{T_0}^{\Fint}$ for any type
  $T_0$ defined in $\ShexSch$ different from $T$. A \emph{flat-referential}
  source-to-target dependency of a strongly typed $\DES$ is of the form
\begin{equation}
  \label{eq:flat-ref-std}
  R(x,y) \rightarrow \Triple(f_T(x), p, f_{T_0}(y)) \land
  T(f_T(x)) \land T_0(f_{T_0}(y)),
  \tag{$\star_{\mathit{ref}}$}
\end{equation}
where $T$ and $T_0$ are types defined by $\ShexSch$, and $p$ is a
property. A \emph{flat-value} source-to-target dependency of a
typed $\DES$ is of the form
\begin{equation}
  \label{eq:flat-val-std}
  R(x,y) \rightarrow \Triple(f_T(x), p, y) \land
  T(f_T(x)) \land S(y),
  \tag{$\star_{\mathit{val}}$}
\end{equation}
where $T$ is a type defined by $\ShexSch$ and $p$ is a property and
$S\in\{\StrSym,\IntSym\}$. A source-to-target dependency is \emph{flat} if it is
either flat-value or flat-referential source to target dependency. For a flat
rule $\sigma$ we set $\relname(\sigma)=R$, $\sourcetype(\sigma)=T$,
$\prop(\sigma)=p$, and $\targettype(\sigma)=T'$ for \eqref{eq:flat-ref-std}
and $\targettype(\sigma)=S$ for \eqref{eq:flat-val-std}. $\DES$ is
\emph{flat} if it is strongly-typed and it uses only flat source-to-target
dependencies.

  }

  \joseinline{

    A shape expression schema $\ShexSch$ defines a containment relation on types
    $T\sqsubseteq T_0$ iff for every graph that is valid w.r.t.\ $\ShexSch$
    every node of type $T$ also has a type $T_0$. We additionally introduce the
    \emph{universal} type $\top_\forall$ (that is not necessarily defined in
    $\ShexSch$) which is satisfied by every node (and consequently, it contains
    every other type). Now, we write $\delta(T,p)=T_0$ with
    $\delta^\mult(T,p)=M$ if $p\dbl T_0^M\in\delta(T)$, and
    $\delta(T,p)=\top_\forall$ with $\delta^\mult(T,p)=\MANY$ if
    $p\dbl T_0^M\not\in\delta(T)$ for any $T$ and $M$.

    A rule $\sigma$ of a flat $\DES$ is \emph{ShEx-compatible} iff
    $\targettype(\sigma)\sqsubseteq\delta(\sourcetype(\sigma),\prop(\sigma))$. A flat
    $\DES$ is \emph{ShEx-consistent} iff for every rule $\sigma$ such that
    $\sigma$ is ShEx-compatible and \\
    $\delta^\mult(\sourcetype(\sigma),\prop(\sigma))\in\{\ONE,\MAYBE\}$, there
    is a key dependency on the relation name $\relname(\sigma)$ on the first
    attribute, and furthermore, there is no other rule in $\stdep$ with the same
    source type symbol and the same property as $\sigma$.

    The following lemma was stated and proved in \cite{fagin:2005a}.
    \begin{lemma}
      \label{lem:homomorphism}
      Let $K_1\cstep{\sigma,h} K_2$ be a chase
      step where $K_2\not=\bot$. Let $K$ be an instance such that: (i) $K$
      satisfies $\sigma$ and (ii) there exists a homomorphism $h_1:K_1 \to
      K$. Then there exists a homomorphism $h_2:K_2 \to K$.
    \end{lemma}

    We denote by $\mathrm{CT}^c_\exists$ the class of set of dependencies such
    that for every database there is a terminating $c$-chase sequence.

    \begin{lemma}
      \label{lem:finite}
      For any flat and skolemized data exchange setting $\DES$, given an
      instance $I$ of schema $\Rsch$, the chase of $I$ with
      $\stdep\cup\Sigma_\ShexSch$ terminates.
    \end{lemma}

    \begin{proof}
      It is shown in \cite{calautti:2016b} that semi-acyclic dependencies belongs
      to the termination class $\mathrm{CT}_\exists^{\mathrm{std}}$. By applying
      the adornment algorithm of \cite{calautti:2016b}, the set of dependencies
      $\stdep\cup\Sigma_\ShexSch$ belong to the class of semi-acyclic dependencies,
      i.e. the chase of $I$ with $\stdep\cup\Sigma_\ShexSch$
      terminates.\qed
    \end{proof}

    \begin{lemma}
      \label{lem-fails}
      For any flat and skolemized data exchange setting $\DES$, given an instance
      $I$ of schema $\Rsch$, the chase of $I$ with
      $\stdep\cup\Sigma_\ShexSch$ fails iff $\solutions(I,\DES)=\emptyset$.
    \end{lemma}

    \begin{proof}
      Take an skolemized data exchange setting $\DES$. Take an instance $I$ of
      schema $\Rsch$.  $(\implies)$ Assume chase of $(I,\emptyset)$ with
      $\stdep\cup\Sigma_\ShexSch$ fails, i.e. the last chase step is not
      performed. Then $\sigma$ for the last chase step must be of the form
      $\varphi\rightarrow x_1=x_2$, and $h:\body(\sigma)\to J$ is a homomorphism
      such that $h(x_1)$ and $h(x_2)$ are two distinct constants $c_1$ and,
      respectively, $c_2$. Suppose that there exists a solution $J'$. Moreover,
      the identity mapping $\mathit{id} : (I,\emptyset)\to (I,J')$ is a homomorphism. By
      lemma \ref{lem:homomorphism}, the existence of a homomorphism
      $g :(I,J) \to (I,J')$. Then $g\circ h:\body(\sigma)\to J'$ is
      a homomorphism. Since $J'$ is assumed to satisfy $\sigma$, it must be the
      case that $g(h(x_1))=g(h(x_2))$ and thus $g(c_1)=g(c_2)$. Homomorphisms
      are identities on $\D$, and so $c_1=c_2$, which is a contradiction.
      $(\impliedby)$ We will prove by contrapositive. Assume chase of
      $(I,\emptyset)$ with $\stdep\cup\Sigma_\ShexSch$ does not fail. By lemma
      \ref{lem:finite}, the chase of $(I,\emptyset)$ with $\stdep\cup\Sigma_\ShexSch$
      terminates and by definition of chase when it finishes, the result is
      a solution. Thus, $\solutions(I,\DES)\not=\emptyset$. \qed
    \end{proof}
    \begin{theorem}
      \label{th:binaryconsistent}
      A flat and decomposed relational to RDF data exchange setting is universally
      consistent if and only if it is ShEx-consistent.
    \end{theorem}
    \begin{proof}
      Take a flat and decomposed relational to RDF data exchange setting\\
      $\DES=(\Rsch,\ShexSch,\stdep,\Fsig,\Fint)$. ($\implies$) We will prove by
      contrapositive. Assume $\DES$ is not ShEx-consistent. Let $\sigma$ be
      a rule of the form
  \[
    R(x,y)\rightarrow T(f_T(x),p_0,f_{T_0}(y)) \land T(f_T(x)) \land
    T_0(f_{T_0}(y))
  \]
  where
  $\targettype(\sigma)\sqsubseteq\delta(\sourcetype(\sigma),\prop(\sigma))$ and
  $\delta^\mult(\sourcetype(\sigma),\prop(\sigma))\in\{\ONE,\MAYBE\}$ and there
  is no key dependency on the relation name $\relname(\sigma)$ or there is
  another rule $\sigma'$ such that source type symbol and property is the same
  as $\sigma$. Then, there are two cases.

  Case 1 When there is not a key dependency on the relation name
  $\relname(\sigma)$. Take a database instance $I(R)=\{(2,1),(2,2)$. By
  condition $\delta^\mult(\sourcetype(\sigma),\prop(\sigma))\in\{\ONE,\MAYBE\}$,
  there is a triple constraint with multiplicity in $\{\ONE,\MAYBE\}$ in the
  type definition of $T$. Let the triple constraint be $p\dbl T_0^1$. By
  lemma~\ref{lem:triple-constraint}, let $\Sigma_\ShexSch$ be the encoding of
  the triple constraint. The chase of $(I,\emptyset)$ with $\stdep$ generates
  $G_0=\{(\mathord{:}2,p_0,1),(\mathord{:}2,p_0,2),(\mathord{:}2,T),\\ (1,T_0),(2,T_0)\}$. Then
  the chase of $(G_0,\emptyset)$ with $\Sigma_\ShexSch$ fails. Thus, the chase
  of $(I,\emptyset)$ with $\stdep\cup\Sigma_\ShexSch$ fails. By lemma
  \ref{lem-fails}, $\solutions(I,\DES)=\emptyset$, then $\DES$ is not
  universally consistent.

  Case 2 When there is another rule $\sigma' \in\stdep$ with the same source and
  property as $\sigma$ of the form
  \begin{align*}
    &R'(x,y)\rightarrow T(f_T(x),p_0,f_{T_0}(y))
      \land T(f_T(x)) \land  T_0(f_{T_0}(y))
  \end{align*}
  Take a database instance $I(R)=\{(2,1)\}$ and $I(R')=\{(2,2)\}$. As in case 1,
  there is a triple constraint with multiplicity one or maybe in the type
  definition of $T$. Let the triple constraint be $p\dbl T_0^1$. By
  \ref{lem:triple-constraint}, let $\Sigma_\ShexSch$ be the encoding of the
  triple constraint. The chase of $(I,\emptyset)$ with $\stdep$ generates
  $G_0=\{(\mathord{:}2,p_0,1),(\mathord{:}2,p_0,2),(\mathord{:}2,T),(1,T_0),(2,T_0)\}$. A similar
  argument of case 1 can be used. Thus $\solutions(I,\DES)=\emptyset$, then
  $\DES$ is not universally consistent.

  ($\impliedby$) Assume $\DES$ is ShEx-consistent. We will prove by
  contradiction. Suppose $\DES$ is not universally consistent, i.e. there is an
  instance $I$ such that $\solutions(I,\DES)=\emptyset$. By lemma
  \ref{lem-fails}, the chase of $(I,\emptyset)$ with $\stdep\cup\Sigma_\ShexSch$
  fails. The chase fails when there is a chase sequence that fails. Thus, there
  is a chase step that can not be performed. Let the chase sequence be as
    $I\cup G_0 \cstep{\sigma_0,h}\ldots
    G_j\cstep{\sigma_j,h}\ldots G_i\cstep{\sigma_i,h}\ldots
    G_k\cstep{\sigma_k,h}\bot$ where $\sigma_k$ is of the form
    $T(x)\land \Triple(x,p,y) \land \Triple(x,p,y') \rightarrow y=y'$ and there is
    a homomorphism $h$ from $\body(\sigma_k)\to G_k$ such that
    $h(y)\not=h(y')$.

  Then,
  \begin{align*}
    T(f_T(h(x)),p,h(y)) \in G_k \land  T(f_T(h(x)),p,h(y)) \in G_{i+1} \land\\
    T(f_T(h(x)),p,h(y)) \not\in G_x , \text{where}\ x\leq i\\
    T(f_T(h(x)),p,h(y')) \in G_k \land  T(f_T(h(x)),p,h(y')) \in G_{j+1} \land\\
    T(f_T(h(x)),p,h(y')) \not\in G_x , \text{where} \ x\leq j\\
%    T(h(x)) \in I_j \land T(h(x)) \not\in I_x, \text{where} \ x<j
  \end{align*}

  We have the following scenarios where $T(f_T(h(x)),p,h(y)) \in G_{i+1}$ and \\
  $T(f_T(h(x)),p,h(y'))\in G_{j+1}$ has been generated.

  \begin{itemize}
  \item When $G_{i+1}$ was the result of applying $\sigma_i$ of the form
    $R(x,y)\rightarrow T(f_T(x),p,y) \land T(f_T(x))$, and when $G_{j+1}$ was
    the result of applying $\sigma_j$ of the form
    $R'(x,y)\rightarrow T(f_T(x),p,y)\land T(f_T(x))$. Then there were an
    homomorphism $h_i$ from $\body(\sigma_i)\to I$ and $h_j$ from
    $\body(\sigma_j)\to I$ such that $h_i(x)=h_j(x)$ and
    $h_i(y)\not=h_j(y)$. Thus, the chase step can not be performed. But then, we
    will have that $\sigma_j$ has the same source type symbol and the same
    property as $\sigma_i$. Then, $\DES$ is not ShEx-consistent, which is
    a contradiction.
  \item When $G_{i+1}$ and $G_{j+1}$ was the result of applying $\sigma_i$, and
    $\sigma_j$ both of them a source-to-target dependency, where
    $\sigma_i=\sigma_j$. Then there were an homomorphism $h_i$ from
    $\body(\sigma_i)\to I$ and $h_j$ from $\body(\sigma_j)\to I$ such that
    $h_i(x)=h_j(x)$ and $h_i(y)\not=h_j(y)$. Thus, the chase step can not be
    performed. But, it will imply that there is not key dependency on
    $\relname(\sigma_i)$. Then $\DES$ is not ShEx-consistent, which is
    a contradiction.
  \item When $G_{i+1}$ and $G_{j+1}$ were the result of applying $\sigma_i$, and
    $\sigma_j$ of the form $\varphi(\bar{y})\rightarrow y_1=y_2$. Since, they
    refer to the same type, then $\sigma_i=\sigma_j$. Consequently, the
    homomorphisms $h_i$ and $h_j$ from $\body(\sigma_i)\to G_i$ and
    $\body(\sigma_j)\to G_j$ respectively were the same
    $h_i(y_1)=h_j(y_1)$. Then there is no contradiction.
  \item When $G_{i+1}$ and $G_{j+1}$ were the result of applying $\sigma_i$, and
    $\sigma_j$ of the form $T(x)\rightarrow \exists y.\ T(x,p,y)$. Then there
    were an homomorphism $h_i$ from $\body(\sigma_i)\to G_i$ and $h_j$ from
    $\body(\sigma_j)\to G_j$ such that $h_i(x)=h_j(x)$ and
    $\bot_1=h_i(y)\not=h_j(y)=\bot_2$. But $\bot_1=\bot_2$ does not generate
    a failure, because when we equate two fresh null constants, the null
    constant of greater index is replaced by the less index.
  \item When $G_{i+1}$ was the result of applying $\sigma_i$ a source-to-target
    dependency, and $G_{j+1}$ was the result of applying $\sigma_j$ of the form
    $T(x)\rightarrow \exists y.\ T(x,p,y)$, where $p$ was a missing
    property. Then there were an homomorphism $h_i$ from
    $\body(\sigma_i)\to G_i$ and $h_j$ from $\body(\sigma_j)\to G_j$ such that
    $c=h_i(y)=h_j(y)=\bot$. Then there is no contradiction.
  \item When $G_{i+1}$ was the result of applying $\sigma_i$ a equality
    generating dependency, and $G_{j+1}$ was the result of applying $\sigma_j$
    of the form $T(x)\rightarrow \exists y.\ T(x,p,y)$. Then there were an
    homomorphism $h_i$ from $\body(\sigma_i)\to G_i$ and $h_j$ from
    $\body(\sigma_j)\to G_j$ such that such that $c=h_i(y)=h_j(y)=\bot$, where
    there is no contradiction.
  \item When $G_{i+1}$ was the result of applying $\sigma_i$ of the form
    $\varphi(\bar{y})\rightarrow y_1=y_2$, and $G_{j+1}$ was the result of
    applying $\sigma_j$ of the form
    $R(x,y) \rightarrow T(f_T(x),p,f_{T_1}(y)) \land T(f_T(x))\land
    T_1(f_{T_1}(y))$, where
    $\targettype(\sigma_i)\not\sqsubseteq\delta(\sourcetype(\sigma_i),\prop(\sigma_i))$.
    Then there were an homomorphism $h_i$ from $\body(\sigma_i)\to G_i$ such
    that $f_{T_2}(h_i(y_1))=f_{T_2}(h_i(y_2))$; and an homomorphism $h_j$ from
    $\body(\sigma_j)\to I$ such that $h_j(y)=c_1$, where $=c_1$ is a constant
    value. But $f_{T_1}(h_i(y_1))\not=f_{T_2}(h_j(y))$ because $f_{T_1}$ and
    $f_{T_2}$ are disjoint functions. Then, the chase step can not be
    performed. Thus, $\sigma_j$ is not ShEx-compatible and consequently, $\DES$
    is not ShEx-consistent, which is a contradiction.
  \end{itemize}
  Consequently, there were cases where the chase sequence failed, then $\DES$ is
  universally consistent.

  \qed
\end{proof}
}


==> tikzconfig.tex <==
\makeatletter
\newdimen\multi@col@width
\newdimen\multi@col@margin
\newcount\multi@col@count
\multi@col@width=0pt

\tikzset{
  multicol/.code={%
    \global\multi@col@count=#1\relax
    \global\let\orig@pgfmatrixendcode=\pgfmatrixendcode
    \global\let\orig@pgfmatrixemptycode=\pgfmatrixemptycode
    \def\pgfmatrixendcode##1{\orig@pgfmatrixendcode%
      ##1%
      \pgfutil@tempdima=\pgf@picmaxx
      \global\multi@col@margin=\pgf@picminx
      \advance\pgfutil@tempdima by -\pgf@picminx
      \divide\pgfutil@tempdima by #1\relax
      \global\multi@col@width=\pgfutil@tempdima
      \pgf@picmaxx=.5\multi@col@width
      \pgf@picminx=-.5\multi@col@width
      \global\pgf@picmaxx=\pgf@picmaxx
      \global\pgf@picminx=\pgf@picminx
      \gdef\multi@adjust@position{%
        \setbox\pgf@matrix@cell=\hbox\bgroup
        \hfil\hskip-1.5\multi@col@margin
        \hfil\hskip-.5\multi@col@width
        \box\pgf@matrix@cell
        \egroup
      }%
      \gdef\multi@temp{\aftergroup\multi@adjust@position}%
      \aftergroup\multi@temp
    }
    \gdef\pgfmatrixemptycode{%
      \orig@pgfmatrixemptycode
      \global\advance\multi@col@count by -1\relax
      \global\pgf@picmaxx=.5\multi@col@width
      \global\pgf@picminx=-.5\multi@col@width
      \ifnum\multi@col@count=1\relax
       \global\let\pgfmatrixemptycode=\orig@pgfmatrixemptycode
      \fi
    }
  }
}
\makeatother
